Whole-Herd Elephant Pose Estimation from Drone Data for Collective Behavior Analysis

This research represents a pioneering application of automated pose estimation from drone data to study elephant behavior in the wild, utilizing video footage captured from Samburu National Reserve, Kenya. The study evaluates two pose estimation workflows: DeepLabCut, known for its application in laboratory settings and emerging wildlife fieldwork, and YOLO-NAS-Pose, a newly released pose estimation model not previously applied to wildlife behavioral studies. These models are trained to analyze elephant herd behavior, focusing on low-resolution ($\sim$50 pixels) subjects to detect key points such as the head, spine, and ears of multiple elephants within a frame. Both workflows demonstrated acceptable quality of pose estimation on the test set, facilitating the automated detection of basic behaviors crucial for studying elephant herd dynamics. For the metrics selected for pose estimation evaluation on the test set -- root mean square error (RMSE), percentage of correct keypoints (PCK), and object keypoint similarity (OKS) -- the YOLO-NAS-Pose workflow outperformed DeepLabCut. Additionally, YOLO-NAS-Pose exceeded DeepLabCut in object detection evaluation. This approach introduces a novel method for wildlife behavioral research, including the burgeoning field of wildlife drone monitoring, with significant implications for wildlife conservation.

==> sec/supplementary_smallds_dlc.tex <==

% Side experiment -- smaller training dataset.  I will omit for now
%To train DeepLabCut, two methods were explored. In the first, 5 frames from each video were selected using K-means quantization-based extraction \cite{Vector2023} and were manually annotated with the keypoints shown in Figure 1. This results in a training dataset of 105 labeled pose patches. DeepLabCut was fine-tuned on this dataset for 100 epochs. DeepLabCut is known for its efficiency with small datasets, so this dataset size may be sufficient \cite{Mathis2018-jg}. 

% ok I'll omit this but here's the values for it's performance in this table.. the val and the test are for these nets. 
% This network works well on val (same video, different frame) but poorly on test. It's worth noting though cause it's a 100 labels instead of 1400, so that's nice.. 

\begin{table*}[ht]
    \centering
    \begin{tabular}{cccccccccc} % Seven columns, all centered
        \hline
        & \multicolumn{3}{c}{DeepLabCut (Val) } & \multicolumn{3}{c}{DeepLabCut (Test) } & \multicolumn{3}{c}{YOLO-NAS-Pose} \\
        \hline
        & RMSE & PCK & OKS & RMSE & PCK & OKS & RMSE & PCK & OKS \\ % Header row
        \hline
        forehead & 2.43 & 64.7 & 0.81 & 35.4 & 1.50 & 0.05 & 20.12 & 0.0 & 0.02 \\    % Data row 1
        ear\_base\_l & 2.16 & 76.4 & 0.85 & 1.50 & 6.01 & 0.08 & 3.11 & 68.7 & 0.84 \\    % Data row 2
        ear\_base\_r & 2.29 & 70.6 & 0.84 & 26.4 & 3.01 & 0.07 & 2.34 & 63.9 & 0.85 \\    % Data row 3
        skull\_base & 1.99 & 58.8 & 0.86 & 23.1 & 3.76 & 2.98 & 0.08 & 64.5 & 0.82 \\    % Data row 4
        shoulders & 2.63 & 23.6 & 0.77 & 11.8 & 5.26 & 3.94 & 0.16 & 40.4 & 0.72 \\    % Data row 5
        hips & 4.32 & 17.6 & 0.59  & 34.4 & 0 & 0.02 &3.22 & 67.5 & 0.82 \\    % Data row 6
        ear\_tip\_l & 2.88 & 47.1 & 0.76 & 21.9 & 3.00 & 0.08 & 3.50 & 47.0 & 0.75 \\    % Data row 7
        ear\_tip\_r & 3.07 & 35.3 & 0.72 & 20.2 & 3.76 & 0.06 & 3.36 & 53.6 & 0.75 \\    % Data row 8
        Average & \textbf{2.72} & \textbf{49.3} & \textbf{0.78} & \textbf{25.0} & \textbf{3.29} & \textbf{0.07} & \textbf{5.32} & \textbf{50.7} & \textbf{0.70} \\ % Data row 9
        \hline
    \end{tabular}
    \caption{Performance metrics of DeepLabCut and YOLO-NAS-Pose models on the test set. Due to the low performance of DeepLabCut on the test set, the validation set was also included.}
    \label{tab:pose_metrics}
\end{table*}

% discussion 
DeepLabCut, when compared to YOLO-NAS-Pose, exhibited signs of severe overfitting, as evidenced by the discrepancy between its performance on validation and test metrics.

While DeepLabCut demonstrated satisfactory qualitative results in labeling a full video from the validation set—where only a few frames were part of the training data—the overfitting issue remains significant. The validation and training datasets were composed of mixed frames from the same videos, leading to an over-generalization to those specific scenarios. 

However, in similar but distinct environments, DeepLabCut struggled. To mitigate this, future work should ensure that training and validation datasets are derived from different videos and locations, enhancing the network's ability to generalize.
